Bijective proofs for Eulerian numbers of types B and D

Let $\Bigl\langle\matrix{n\cr k}\Bigr\rangle$, $\Bigl\langle\matrix{B_n\cr k}\Bigr\rangle$, and $\Bigl\langle\matrix{D_n\cr k}\Bigr\rangle$ be the Eulerian numbers in the types A, B, and D, respectively -- that is, the number of permutations of n elements with $k$ descents, the number of signed permutations (of $n$ elements) with $k$ type B descents, the number of even signed permutations (of $n$ elements) with $k$ type D descents. Let $S_n(t) = \sum_{k = 0}^{n-1} \Bigl\langle\matrix{n\cr k}\Bigr\rangle t^k$, $B_n(t) = \sum_{k = 0}^n \Bigl\langle\matrix{B_n\cr k}\Bigr\rangle t^k$, and $D_n(t) = \sum_{k = 0}^n \Bigl\langle\matrix{D_n\cr k}\Bigr\rangle t^k$. We give bijective proofs of the identity $$B_n(t^2) = (1 + t)^{n+1}S_n(t) - 2^n tS_n(t^2)$$ and of Stembridge's identity $$D_n(t) = B_n(t) - n2^{n-1}tS_{n-1}(t).$$ These bijective proofs rely on a representation of signed permutations as paths. Using this representation we also establish a bijective correspondence between even signed permutations and pairs $(w, E)$ with $([n], E)$ a threshold graph and $w$ a degree ordering of $([n], E)$, which we use to obtain bijective proofs of enumerative results for threshold graphs.

==> macros.tex <==
\RequirePackage{xspace}
\RequirePackage{mytheorems}
\RequirePackage{paralist}
\RequirePackage{xcolor}

\newcommand{\mybar}[1]{\;\textcolor{#1}{\rule{1pt}{8pt}}\;}
\newcommand{\set}[1]{\{\,#1\,\}}
\newcommand{\upair}[1]{\{#1\}}
\newcommand{\pair}[1]{(#1)}
\newcommand{\bbar}{\mybar{blue}}
\newcommand{\gbar}{\mybar{green}}

\newcommand{\bbp}{bibarred permutation\xspace}
\newcommand{\eul}[2]{\left \langle 
    \begin{array}{@{}c@{}}
      #1 \\ #2
    \end{array}
\right\rangle}

\newcommand{\smallEul}[2]{\left\langle
    \scriptsize
    \begin{array}{@{}c@{}}
      #1 \\ #2
    \end{array}
  \right\rangle}


\newcommand{\stirling}[2]{\left \{ 
    \begin{array}{@{}c@{}}
      #1 \\ #2
    \end{array}
\right\}}

\newcommand{\smallStirling}[2]{\left \{
    \scriptsize
    \begin{array}{@{}c@{}}
        #1 \\ #2
      \end{array}
    \right\}}


\newcommand{\A}{\ensuremath{\mathsf{A}}}
\newcommand{\B}{\ensuremath{\mathsf{B}}}
\newcommand{\D}{\ensuremath{\mathsf{D}}}

\newcommand{\eulA}[2]{\eul{#1}{#2}}
\newcommand{\eulB}[2]{\eul{\B_{#1}}{#2}}
\newcommand{\eulBb}[2]{\eul{#1}{#2}_{\!\!\overline{\B}}}
\newcommand{\eulD}[2]{\eul{\D_{#1}}{#2}}

\newcommand{\sEulA}[2]{\smallEul{#1}{#2}}
\newcommand{\sEulB}[2]{\smallEul{\B_{#1}}{#2}}
\newcommand{\sEulBb}[2]{\smallEul{#1}{#2}_{\!\!\overline{\B}}}
\newcommand{\sEulD}[2]{\smallEul{\D_{#1}}{#2}}

\DeclareMathOperator{\card}{card}
\newcommand{\Card}[1]{|#1|}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceiling}[1]{\left\lceil #1 \right\rceil}
\newcommand{\xiD}[1][D]{\xi_{#1}}
\newcommand{\MyExpr}[1]{\ceiling{\frac{\Card{\xiD(#1)}}{2}}}
\newcommand{\Myexpr}[1]{\ceiling{\frac{\Card{#1}}{2}}}
\newcommand{\rto}[1][\quad]{\xrightarrow{#1}}
\newcommand{\eqdef}{:=}
\newcommand{\des}[2][]{\mathrm{des}_{#1}(#2)}
\newcommand{\Desc}[2][]{\mathrm{Des}_{#1}(#2)}
\newcommand{\desc}[2][]{\Desc[#1]{#2}}
\newcommand{\inv}[2][]{\mathrm{Inv}_{#1}(#2)}
\newcommand{\invB}[2][]{\inv[\B]{#2}}
\newcommand{\invD}[2][]{\inv[\D]{#2}}
\newcommand{\DescB}[1]{\Desc[\B]{#1}}
\newcommand{\descB}[1]{\desc[\B]{#1}}
\newcommand{\descBp}[1]{\mathrm{Des}_{\B}^{+}(#1)}
\newcommand{\desB}[1]{\des[\B]{#1}}
\newcommand{\descD}[1]{\desc[\D]{#1}}
\newcommand{\DescD}[1]{\Desc[\D]{#1}}
\newcommand{\desD}[1]{\des[\D]{#1}}
\newcommand{\descp}[2][]{D^{+}_{#1}(#2)}
\newcommand{\descm}[2][]{D^{-}_{#1}(#2)}
\newcommand{\descn}[2][]{\descm[#1]{#2}}
\newcommand{\descpos}[2][]{D_{> 0}(#2)}
\newcommand{\sbp}{simply barred permutation\xspace}
\newcommand{\wbp}{loosely barred permutation\xspace}
\newcommand{\Wbp}{Loosely barred permutation\xspace}
\renewcommand{\sp}{signed permutation\xspace}
\newcommand{\Sp}{Signed permutation\xspace}
\newcommand{\esp}{even-\sp}
\newcommand{\fsp}{forked \sp}
\newcommand{\vbar}{|}
\newcommand{\wbar}[1]{\overline{#1}}
\newcommand{\simpl}{\varsigma}
\newcommand{\myexpr}[1]{\ceiling{\frac{\Card{#1}}{2}}}
\newcommand{\SBP}{\mathtt{SBP}}
\newcommand{\SBPn}{\mathtt{SBP}_{n}}
\newcommand{\SBPnk}[1][k]{\mathtt{SBP}_{n,#1}}
\newcommand{\WBP}{\mathtt{LBP}}
\newcommand{\WBPn}{\WBP_{n}}
\newcommand{\WBPnk}[1][k]{\WBP_{n,#1}}
\newcommand{\tiff}{\text{ iff }}
\newcommand{\Tiff}{\quad\text{ iff }\quad}
\newcommand{\tor}{\text{ or }}
\newcommand{\tand}{\text{ and }}

\newcommand{\setn}[1][n]{[#1]}
\newcommand{\setnp}[1][n]{[#1]_{0}}
\newcommand{\setpmn}[1][n]{[\pm #1]}
\newcommand{\setmn}{[-n]}
\newcommand{\Perm}{\mathsf{P}}
\newcommand{\Sg}{\mathsf{S}}
\newcommand{\Pn}{\Perm_{\!n\,}}
\newcommand{\Sn}{\Sg_{n}}
\newcommand{\Bn}{\B_{n}}
\newcommand{\Dn}{\D_{n}}

\newcommand{\HBn}{\mathcal{H}(\Bn)}
\newcommand{\HDn}{\mathcal{H}(\Dn)}

\newcommand{\abs}[1]{|#1|}
\newcommand{\jirr}{join-irreducible\xspace}
\newcommand{\smooth}{smooth\xspace}
\newcommand{\ns}{non-\smooth}
\newcommand{\mate}[1]{\underline{#1}}
\RequirePackage{accents}
\DeclareMathAccent{\wtilde}{\mathord}{largesymbols}{"65}
\newcommand{\lowermate}[1]{\underaccent{\wtilde}{#1}}

\newcommand{\EndOfExample}{\EndOfRemark}
\newcommand{\glrepr}{grid-like representation\xspace}
\newcommand{\ad}{anti-diagonal\xspace}
\newcommand{\xyturn}{East-South turn\xspace}

\newcommand{\En}{Eulerian number\xspace}
\newcommand{\Ep}{Eulerian polynomial\xspace}
\newcommand{\Stem}{Stembridge\xspace}
\newcommand{\StemI}{\Stem's identity\xspace}
\newcommand{\resp}{resp.,\xspace}
\newcommand{\prep}{path representation\xspace}
\newcommand{\Prep}{Path representation\xspace}
\newcommand{\Es}{East step\xspace}
\newcommand{\Ss}{South step\xspace}

\newcommand{\ESs}{East and South step\xspace}

\newenvironment{ex}{\begin{example}}{\EndOfExample\end{example}}

\newcommand{\tg}{threshold graph\xspace}
\newcommand{\Tg}{Threshold graph\xspace}
\newcommand{\dgo}{degree ordering\xspace}
\newcommand{\cdgo}{canonical \dgo}
\newcommand{\ap}{\red{annotated permutation}\xspace}
\newcommand{\lw}{<_{w}}
\newcommand{\leqw}{\leq_{w}}
\newcommand{\contr}{contradiction\xspace}
\newcommand{\vp}[1][]{\mathrel{\lhd_{#1}}}
\newcommand{\vpE}{\vp[E]}
\newcommand{\VP}[3][E]{\NE[#1](#2) \subseteq \SE[#1]{#3}}
\newcommand{\NE}[1][E]{N_{#1}}
\newcommand{\SE}[2][E]{N_{#1}[#2]}
\newcommand{\degE}[1][E]{\deg_{#1}}

\newcommand{\sa}{self-adjoint\xspace}
\newcommand{\fp}{fixed point\xspace}
\newcommand{\fpf}{fixed-point-free\xspace}
\newcommand{\hf}{height function\xspace}
\newcommand{\fpfsaGc}{\fpf \sa Galois connection\xspace}
\newcommand{\fpfsahf}{\fpf \sa \hf}
\newcommand{\Eu}[1][u]{E^{#1}}

\newcommand{\luy}{\ensuremath{\lambda^{u}_{\mathtt{y}}}}
\newcommand{\lux}[1][u]{\ensuremath{\lambda^{#1}_{\mathtt{x}}}}
\newcommand{\minus}[1]{-#1}

\newcommand{\thetan}[1][n]{\theta_{#1}}

\newcommand{\ts}{threshold\xspace}
\newcommand{\tsg}{\ts graph\xspace}
\newcommand{\height}{\mathrm{height}}
\newcommand{\width}{\mathrm{width}}

\newcommand{\Pin}{\mathsf{Pi}^{+}_{\mathtt{E,S}}(\setnp,\setnp)} 
\newcommand{\GCn}{\mathsf{GC}_{\mathtt{fpfsa}}(\setnp)} 
\newcommand{\HFn}{\mathsf{HF}_{\mathtt{fpfsa}}(\setnp)} 
\newcommand{\TGn}{\mathsf{TG}^\mathtt{dgo}_{n}} 

\newcommand{\Img}{Im}



\newcommand{\es}{even signed}

\newcommand{\Gc}{Galois connection\xspace}

\renewcommand{\fact}[1]{#1!}

\newcommand{\normal}{normal\xspace}
\newcommand{\antidiagonal}{antidiagonal\xspace}
\newcommand{\vertices}{vertices\xspace}


